A Replication Study: Machine Learning Models Are Capable of Predicting Sexual Orientation From Facial Images

Recent research used machine learning methods to predict a person's sexual orientation from their photograph (Wang and Kosinski, 2017). To verify this result, two of these models are replicated, one based on a deep neural network (DNN) and one on facial morphology (FM). Using a new dataset of 20,910 photographs from dating websites, the ability to predict sexual orientation is confirmed (DNN accuracy male 68%, female 77%, FM male 62%, female 72%). To investigate whether facial features such as brightness or predominant colours are predictive of sexual orientation, a new model based on highly blurred facial images was created. This model was also able to predict sexual orientation (male 63%, female 72%). The tested models are invariant to intentional changes to a subject's makeup, eyewear, facial hair and head pose (angle that the photograph is taken at). It is shown that the head pose is not correlated with sexual orientation. While demonstrating that dating profile images carry rich information about sexual orientation these results leave open the question of how much is determined by facial morphology and how much by differences in grooming, presentation and lifestyle. The advent of new technology that is able to detect sexual orientation in this way may have serious implications for the privacy and safety of gay men and women.

==> chapters/chapter1/main.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\chapter{The First Chapter}
\label{chap:first}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Explain what the chapter focusses on. Be brief, and only focus on the main theme of the chapter. Also reference any previous chapters that link to the theme of this chapter.

Then, outline the remaining sections and what each covers in a broad sense. Use labeled references like these: Section~\ref{sec:first:first_sec}, Section~\ref{sec:first:second_sec} and Section~\ref{sec:first:summary}. Note that all labels in this document follow a convention, but you are free to choose whatever labels you want to.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{A First Section}
\label{sec:first:first_sec}

The text may include sections, subsections and sub-subsections. Refer to the ``Not So Short Introduction to \LaTeXe'' for more details on what types of organisation are available to you. Include labels for each section, subsection and sub-sub-section, so that you can easily reference them in your text, as was shown in the previous section (this also ensures that your numbering will still be correct, even if you add additional sections and subsections at a later date). Any undefined labels that you reference will not cause the document build process to fail. Instead, they are replaced by question marks, and will generate warnings while compiling. Watch out for these before you submit work.

Equations are included as follows:
\begin{equation}
\label{eq:eqn}
	\eta(t)=t+c
\end{equation}
Make sure that you define all the symbols you use in your equations. Equations are referenced in the text as follows: Equation~(\ref{eq:eqn}).

\begin{figure}
	\centering{\includegraphics{chapters/chapter1/figures/fig1}}
	\caption[A short caption, for the figure list]{A long caption, for under the figure.}
	\label{fig:fig1}
\end{figure}
You may include figures, such as Figure~\ref{fig:fig1}. Note the short caption has no period at the end of it, while the long caption does (in other words, always provide the short caption without the period, even if the text is the same as the long caption). We recommend using Xfig (which is an open source tool) if you can for your diagrams. Make sure that the files you create are in encapsulated postscript (eps) format. Note that you must not specify the file extension when including the image (this is because PDF generation automatically converts eps image files to PDF files).

\begin{graph}
	\centering{\includegraphics{chapters/chapter1/graphs/graph1}}
	\vspace{10pt}
	\caption[A short graph caption]{A long graph caption.}
	\label{grf:graph1}
\end{graph}
You may also provide graphs, such as Graph~\ref{grf:graph1}. The captions follow the same principal as for figures. We recommend using the very flexible gnuplot (which is open source software) to generate your graphs.

\begin{table}
	\caption[A short table caption]{A long table caption.}
	\centering{
		\begin{tabular}[t]{|l|c|c|}
			\hline
			\textbf{Parameter} & \textbf{Symbol} & \textbf{Domain}    \\
			\hline
			First           & $A$          & $[2,\infty)$    \\
			Second          & $B$    & $[0.0,\infty)$  \\
			Third           & $C$   & $(0.0,\infty)$  \\
		\end{tabular}
	}
	\label{tab:table1}
\end{table}
You may include tables, such as Table~\ref{tab:table1}. The captions follow the same principal as for figures and graphs. You may use a package called \texttt{hhline} to add fancy borders to your tables. Please refer to the package documentation for details.

\begin{algorithm}
	\centering{\fbox{\parbox[]{155mm}{
		\setlength{\parindent}{0.3cm}
		\vspace{0.3cm}
		\small{
		\indent Initialise all variables
		\par\textbf{repeat:}
		\par\hspace{1cm}Select a pattern, and load it
		\par\hspace{1cm}\textbf{for all} {\em values $v$ in the pattern\/} \textbf{do}
		\par\hspace{1cm}\hspace{1cm}Analyse the pattern
		\par\hspace{1cm}\textbf{end for}
		\par\textbf{until} {\em stopping criteria are met}
		}
		\vspace{0.3cm}
	}}}
	\caption[A short algorithm caption]{A long algorithm caption.}
	\label{alg:algorithm1}
\end{algorithm}
Finally, you may add algorithms, such as Algorithm~\ref{alg:algorithm1}. You are free to typeset these as you see fit, or use one of the many algorithm-related packages that are available. In the future, we will try to develop a nice way of generating pseudocode in a standard format like what you see in Algorithm~\ref{alg:algorithm1}. Again, the captioning conventions are the same as for figures, graphs and tables.

All floating bodies (i.e.\ figures, graphs, tables and algorithms) are automatically positioned by \LaTeX. You can change this behaviour by modifying a number of fractions that govern when and where \LaTeX\ can position floating bodies. These are located in \texttt{dissertation.tex}, and there are a several you can modify (e.g.\ \texttt{topfraction}, \texttt{bottomfraction}, \texttt{textfraction} and \texttt{floatpagefraction}). Note that any floating bodies that cannot be placed throughout the text will group together on ``float pages''.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{A Second Section}
\label{sec:first:second_sec}

This is how a second section would appear in your document. You cannot nest sections in one another (to get that effect, use sub-section). It may improve the flow of your writing if you introduce the subsections before jumping into them, so that the reader has an idea of what is coming. Again, use the subsection's labels to ensure that the correct numbering is used throughout.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{A Subsection}
\label{sec:first:second_sec:sub}

You may place subsections as well. Again, these cannot be nested in one another. Consider the overall structure of your dissertation very carefully before writing. Try to avoid too many short subsections, and split your discussion logically between sections and subsections.

\subsubsection{A Sub-Subsection}
\label{sec:first:second_sec:sub:subsub}

You may even add a third level of headings, called sub-subsections (although these are not numbered, or listed on the contents page). It pays to carefully consider whether you will be including sub-subsections. If the text for such a section is short, and there aren't many topics to cover, bulleted lists often look better. However, if the text needs to be broken up into paragraphs, rather use sub-subsections. Also, try to avoid too many sub-subsections, since they cannot be referenced properly, and may become confusing to the reader if they stretch over too many pages. Also, note that while you can label a sub-subsection (just like a section or subsection), referencing the label will simply provide the number of the subsection within which the sub-subsection is located.

You can include acronyms in your dissertation as follows: \useacronym{AI}, \useacronym{ANN} and \useacronym{CI}. The acronyms should all be defined in \texttt{dissertation.tex}, using \texttt{newacronym}. Note that on the first use of the acronym, the full term is used, with the acronym following it in parentheses. On subsequent uses (such as \useacronym{AI}), only the acronym is given.

While it is not at all necessary, you might like to include index terms in your dissertation. You can do this by providing index terms in the text when you mention the topic (e.g.\ widgets\index{Widgets}). You can make an index term bold in the index if it's a primary page reference (e.g.\ for artificial intelligence\index{Artificial Intelligence|idxbf}). If you index the same term again, it will show up as a non-bold secondary reference. You can provide references to other index terms in the \texttt{dissertation.tex} file. There are many more options, but these are outlined properly in the \texttt{makeindx} documentation.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Summary}
\label{sec:first:summary}

This section should follow all the previous ones forming the main body of the chapter. Provide an outline of the previous sections of this chapter, explaining what each dealt with. Provide section references using labels, as you did for the outline at the start of the chapter.

Give a brief synopsis of what the following chapter will cover, in a general sense. This will improve the logical flow of your work from one chapter to the next.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> chapters/chapter2/main.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\chapter{The Second Chapter}
\label{chap:second}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The same structure as before, including section, subsections and sub-subsections. Make sure that you follow the same conventions throughout, to avoid confusing the reader. Always remember to include a summary.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{The First Section}
\label{sec:second:first_sec}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{The Second Section}
\label{sec:second:second_sec}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{A Subsection}
\label{sec:second:second_sec:one}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Another Subsection}
\label{sec:second:second_sec:two}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Summary}
\label{sec:second:summary}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> chapters/conclusions/main.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\chapter{Conclusions}
\label{chap:conclusions}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Provide an introduction, stating that this chapter summarises the conclusions of your work, and consider future directions that related research could take. Again, reference Sections~\ref{sec:conclusions:conclusion_summary} and \ref{sec:conclusions:future_work}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Summary of Conclusions}
\label{sec:conclusions:conclusion_summary}

Summarise your conclusions here. You should consider each of the objectives you listed in the introduction, and explain how each was met, providing a discussion on what your specific findings were for each. Also mention what novel contributions (these might include a new taxonomy, model, algorithm, or empirical results not previously published) your work has introduced to the field while the various objectives were being addressed.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Future Work}
\label{sec:conclusions:future_work}

Enumerate the future work that you could foresee developing from the work you have done here. Mention areas you could not focus on, or possible extensions to your work. It is a good idea to be thorough, since you increase your chances of being referenced by other researchers who follow up on your work, even if you do not do so yourself. You may consider writing this as a bulleted list, if you mention many aspects.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
